Assessing generalisability of deep learning-based polyp detection and segmentation methods through a computer vision challenge

Polyps are well-known cancer precursors identified by colonoscopy. However, variability in their size, location, and surface largely affect identification, localisation, and characterisation. Moreover, colonoscopic surveillance and removal of polyps (referred to as polypectomy ) are highly operator-dependent procedures. There exist a high missed detection rate and incomplete removal of colonic polyps due to their variable nature, the difficulties to delineate the abnormality, the high recurrence rates, and the anatomical topography of the colon. There have been several developments in realising automated methods for both detection and segmentation of these polyps using machine learning. However, the major drawback in most of these methods is their ability to generalise to out-of-sample unseen datasets that come from different centres, modalities and acquisition systems. To test this hypothesis rigorously we curated a multi-centre and multi-population dataset acquired from multiple colonoscopy systems and challenged teams comprising machine learning experts to develop robust automated detection and segmentation methods as part of our crowd-sourcing Endoscopic computer vision challenge (EndoCV) 2021. In this paper, we analyse the detection results of the four top (among seven) teams and the segmentation results of the five top teams (among 16). Our analyses demonstrate that the top-ranking teams concentrated on accuracy (i.e., accuracy > 80% on overall Dice score on different validation sets) over real-time performance required for clinical applicability. We further dissect the methods and provide an experiment-based hypothesis that reveals the need for improved generalisability to tackle diversity present in multi-centre datasets.

==> Disscussion.tex <==
\section*{Discussion}
These will include discussions on what we participants have used, what are the best practices based on results and future direction.
\begin{itemize}
    \item Preprocessing effect
    \item Loss function, model (highlight single stage or 2 stage or combined models) 
    \item Generalization 
    \item Performance (runtime) on GPU and CPU (if available)
    \item Future directions
\end{itemize}

==> EndoCV2021_challenge.tex <==
\section*{The EndoCV challenge: Dataset, evaluation and submission}
% To rewrite the below
In this section, we present the dataset compiled for the polyp generalisation challenge, the protocol used to obtain the ground truth, evaluation metrics that were defined to assess the participants methods and a brief summary on the challenge setup and ranking procedure.
%
\subsection*{Dataset and challenge tasks}
% challenge dataset
% TODO: overview on dataset - describe figure 1  
\paragraph{Dataset:} The EndoCV2021 challenge addresses the generalisability of polyp detection and segmentation tasks in endoscopy frames. The colonoscopy video frames utilised in the challenge are gathered from six different centres including two modalities (i.e. WL and NBI) with both sequence and non-sequence frames (see Fig. \ref{fig:my_label_data} a). The challenge includes five different types of data and participants were allowed to combine accordingly for their train-validation splits: i) multi-centre video frames from five centres for training and validation, ii) polyp size-based, iii) single frame and sequence data split, iv) modality split (i.e. only for testing phase) and v) one hidden centre test (test phase only). The training dataset consisted of a total of 3242 WL frames from five centers (i.e. C1-C5) with both single and sequence frames. For the test dataset, it is comprised of: a) dataset with unseen modality, NBI (data 1), b) dataset with single frames from unknown center (data 2), c) frame sequences from the mixed centers (C1-C5, data 3), and iv) the unseen center sequence frames (C6, data 4). A total of 777 frames were used and data 3 was picked as base dataset against which generalisability of methods were assessed. Polyp size distribution (see Fig. \ref{fig:my_label_data}, left) (b)) and its size in log-scale (see Fig. \ref{fig:my_label_data} (b), right) in both training and test sets are presented. These sizes were divided into null (for no polyp in frames), small ($< 100 \times 100$ pixels bounding box), medium ($\leq200\times200$ pixels polyp bounding box) and large ($> 200\times200$ pixels polyp bounding box).
% TODO: write the number of each size here: check the code
% TODO: talk about deviation on polyp sizes

% Moreover, as shown in Fig \ref{fig:my_label_data} (b) there is a variation in the polyp size in the frames of the provided dataset in addition to the non-polyp frames.

% challenge tasks
% TODO: How test dataset was used and how these challenge tasks were divided - general overview on generalisability
%TODO: Detection challenge - 

\paragraph{Challenge tasks:} EndoCV2021 included two tasks for which the generalisability assessment was also conducted: 1) detection and localisation task and 2) pixel-level segmentation task. For the detection task, participants were provided both single and sequence frames with manually annotated ground truth polyp labels and their corresponding bounding boxes. Participants were required to train their model for predicting class labels, bounding box co-ordinates and confidence scores for localisation. For the segmentation task, we provided the pixel level ground truth segmentation from experts that included the same data as provided for the detection task. Here, the participants were challenged to obtain close to ground truth segmentation binary map prediction. Both of these challenge tasks were assessed rigorously to understand the generalisability of the developed methods. In this regard, the test data consisted of four different categories, here we call it as \textbf{data 1}, \textbf{data 2}, \textbf{data 3} and \textbf{data 4}. Data 1 consisted of unseen modality with narrow-band imaging data (NBI) widely used as multi-modal imaging in colonoscopy, data 2 comprises of single frames of unseen center C6, data 3 consisted of mixed seen center (C1-C5) sequence data and data 4 included sequence data from unseen center C6. For generalisabilty, we compared the scores between data 3 (seen center data) with the other unseen data categories. All test results were evaluated on a common NVIDIA Tesla V100 GPU. Further details on metric computation is provided in Section \textbf{Evaluation metrics}.

% For the detection task, participants were provided with bounding-box frame level annotation for both frame single and sequence images. Each team provided the 
%TODO: Segmenation- - 
% Inference done on cloud GPU V100
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/Test-train_endoCV2021.pdf}
    \caption{\textbf{Multi-center training and test samples:} a. Colonoscopy video frames for which the annotation samples were reviewed and released as training (left) and test (right) is provided. Training samples included nearly proportional frames from five centers (C1-C5) while test samples consist of majority of single and sequence frames from unseen center (C6); b. Number of polyp or non-polyp samples-based on polyp sizes (left) and their intra-size variability (right) for training (top) and testing data (bottom).}
    \label{fig:my_label_data}
\end{figure}
\subsubsection*{Ethical and privacy aspects of the data}
% TODO:
The Data for EndoCV2021 was gathered from 6 different centers located in five different countries  (i.e. UK,  Italy, France, Norway and Egypt). The ethical, legal and privacy of the relevant data was handled by each responsible center. The data collected from each centered included a minimum of two essential steps as described below: 
\begin{itemize}
    \item Patient consenting procedure at each institution (required).
    \item Review of the data collection plan by a local medical ethics committee or an institutional review board.
    \item Anonymization of the video or image frames (including demographic information) before sending to the organizers (required).
\end{itemize}

Table \ref{tab:patientConsentingInfo}  illustrates the ethical and legal processes fulfilled by each center along with the details of the endoscopic equipment and recorders used for the collected data. 
%
\begin{table*}[t!]
\small{
\begin{tabular}{l|l|l|l|l}
\hline
\textbf{Centers}                              & \textbf{System info.}                & \textbf{Ethical approval} & \begin{tabular}[l]{@{}l@{}}\textbf{Patient consent} \\\textbf{type}\end{tabular}  & \begin{tabular}[l]{@{}l@{}}\textbf{Recording} \\\textbf{system}\end{tabular} \\ \hline
\begin{tabular}[l]{@{}l@{}} Ambroise Par\'{e} Hospital,\\Paris, France    \end{tabular}     & Olympus Exera 195              & \begin{tabular}[l]{@{}l@{}} N° IDRCB:\\ 2019-A01602-55\end{tabular}      & Endospectral study &  NA  \\ \hline
\begin{tabular}[l]{@{}l@{}} Istituto Oncologico Veneto,\\ Padova, Italy\end{tabular}	     & Olympus endoscope H190 & NA & \begin{tabular}[l]{@{}l@{}}Generic patients \\consent\end{tabular} & \begin{tabular}[l]{@{}l@{}}ENDOX,\\ TESImaging  \end{tabular} \\ \hline
{{\begin{tabular}[l]{@{}l@{}} Centro Riferimento Oncologico,\\ IRCCS, Italy\end{tabular}}}   &\begin{tabular}[l]{@{}l@{}} Olympus VG-165, CV180, \\H185 \end{tabular}         & NA                        & \begin{tabular}[c]{@{}l@{}}Generic patients \\consent\end{tabular}    &        \\ \hline
\begin{tabular}[l]{@{}l@{}}Oslo University Hospital,\\ Oslo, Norway\end{tabular} & \begin{tabular}[l]{@{}l@{}}Olympus Evis Exera III,\\ CF 190 \end{tabular} &Exempted$^\dag$  & \begin{tabular}[l]{@{}l@{}}Written informed\\ consent\end{tabular}   & Pix-E5    \\ \hline
\begin{tabular}[l]{@{}l@{}}John Radcliffe Hospital, \\Oxford, UK\end{tabular}           & \begin{tabular}[l]{@{}l@{}}GIF-H260Z, EVIS Lucera CV260,\\Olympus Medical Systems\end{tabular} & \begin{tabular}[l]{@{}l@{}}REC Ref: \\16/YH/0247 \end{tabular}& Universal consent & MediCapture
\\ \hline
\begin{tabular}[l]{@{}l@{}}University of Alexandria, \\Alexandria, Egypt\end{tabular} & Olympus Exera 160AL, 180AL                             & NA                        & \begin{tabular}[l]{@{}l@{}}Written informed \\consent\end{tabular}  &   NA   \\ \hline
\multicolumn{5}{l}{$^\dag$ Approved by the data inspectorate. No further ethical approval was required as it did not interfere with patient treatment}
\end{tabular}
}
\caption{\textbf{Data collection information for each center:} Data acquisition system and patient consenting information. \label{tab:patientConsentingInfo}}
\end{table*}

\subsubsection*{Annotation protocol}
% TODO - collection protocol (50 unique patient videos/samples) - curation (any patient information - keeping the original size of the frames - annotation protocol desscribed below - developed jointly be computational expertts and gasttroenterologist - drafted and circulated - itemise )
The annotation process was conducted by a team of three experienced researchers using an online annotation tool called Labelbox\footnote{https://labelbox.com}.
To ensure the correctness of the annotation, each annotation was cross-validated by the team and by the center expert for accurate boundaries segmentation. A senior gastroenterologist was assigned for an independent binary review process. To minimise heterogeneity of the manual delineation process, a set of protocols for manual annotation of polyp has been designed as follows: 

\begin{itemize}
 \item Clear raised polyps: Boundary pixels should include only protruded regions. Precaution has to be taken when delineating along the normal colon folds 
\item Inked polyp regions: Only part of the non-inked appearing object delineation 
\item	Polyps with instrument parts: Annotation should not include instrument and is required to be carefully delineated and may form more than one object 
\item	Pedunculated polyps: Annotation should include all raised regions unless appearing on the fold 
\item	Flat polyps: Zooming the regions identified with flat polyps before manual delineation. Also, consulting center expert if needed. 
\end{itemize}

The annotated masks where examined by experienced gastroenterologists were a binary score was given to evaluate the current annotation if it is considered clinically acceptable or not. Additionally, some of the experts provided feedback on the annotation where these images were placed into an ambiguous category for further refinement based on the experts feedback.

% Please add here as discussed @ Debesh
\subsection*{Evaluation metrics}
% TODO
\subsubsection*{Polyp detection}
For the polyp detection task, we have computed standard computer vision metrics such as average precision (AP) and intersection-of-union (IoU)~\cite{everingham2015pascal,lin2014microsoft}. 

\begin{itemize}
\item {IoU}: The IoU metrics measures the overlap between two bounding boxes A and B as the ratio between the target mask and predicted output.
\begin{equation}
\text{IoU(A,B)} =\frac{A \cap B} {A \cup B} 
\end{equation}
Here, $\cap$ represents intersection and $\cup$ represents the union. \item {AP}: AP is computed as the Area Under Curve (AUC) of the precision-recall curve of detection sampled at all unique recall values (r1, r2, ...) whenever the maximum precision value drops:
\begin{equation}
    \mathrm{AP} = \sum_n{\left\{\left(r_{n+1}-r_{n}\right)p_{\mathrm{interp}}(r_{n+1})\right\}}, 
\end{equation}
with $p_{\mathrm{interp}}(r_{n+1}) =\underset{\tilde{r}\ge r_{n+1}}{\max}p(\tilde{r})$. Here, $p(r_n)$ denotes the precision value at a given recall value. This definition ensures monotonically decreasing precision. AP was computed as an average APs at $0.50$  and $0.95$ with the increment of 0.05. Additionally, we have calculated
APsmall, APmedium, APlarge.  More description about the detection evaluation metrics and their formulas can be found here~\footnote{{https://github.com/sharibox/EndoCV2021-polyp\_det\_seg\_gen/blob/main/evaluationMetrics/coco\_evaluator.py}}. 
\end{itemize}
%
\subsubsection*{Polyp segmentation }
For polyp segmentation task, we have used widely accepted computer vision metrics that include Sørensen–Dice Coefficient ($DSC = \frac{2 \cdot tp} {2 \cdot tp + fp + fn}$), {Jaccard Coefficient} ($JC= \frac{tp} {tp + fp + fn}$), precision ($p=\frac{tp} {tp + fp}$), and recall ($r= \frac{tp} {tp + fn}$), overall accuracy \textit{($Acc = {\frac{tp + tn} {tp + tn + fp + fn}}$ )}, and F2 ($=\frac{5p \times r} {4p + r}$). In addition to the performance metrics, we have also computed frame per second (FPS$ = {\frac{\#frames} {sec}}$). Here,  \textit{tp}, \textit{fp}, \textit{tn}, and fn represent true positives, false positives, true negatives, and false negatives, respectively. 

Another commonly used segmentation metric that is based on the distance between two point sets, here ground truth (G) and estimated or predicted (E) pixels, to estimate ranking errors is the average Hausdorff distance ($H_{d}$) and defined as:
\begin{equation}
    H_{d}(G, E) = \bigg(\frac{1}{G} \sum_{g\in G} \min_{e\in E} d(g, e) + \frac{1}{E} \sum_{e\in E} \min_{g\in G} d (g, e)\bigg)/2.
\end{equation}
% The definition of each metrics and their description can also be found in our previous competition paper~\cite{ali2020objective}. 
\subsubsection*{Polyp generalisation metrics}
%
We define the generalisability score based on the stability of the algorithm performance on seen white light modality and center dataset (data 3) with unseen center split (data 2 and data 4) and unseen modality (data 1) in the test dataset. We conducted the generalisability assessment for both detection and segmentation approaches separately. 

For detection, the deviation in score between seen and unseen data types are computed over different $AP$ categories, $k \in \{mean, small, medium, large\}$ with tolerance, ($tl = 0.1$):
\begin{equation}
    dev\_g = \frac{1}{|k|}\sum_k\begin{cases}
    |(\mathrm{AP_k}^{seen}- tl *\mathrm{AP_k}^{seen})  - \mathrm{AP_k}^{unseen}|, & \text{for } \mathrm{AP_k}^{seen} - tl *\mathrm{AP_k}^{seen}) \leq  \mathrm{AP_k}^{unseen}| \geq \mathrm{AP_k}^{seen} + tl *\mathrm{AP_k}^{seen}\\
                            0, \quad \text{otherwise.} \\
                         \end{cases}
\end{equation}
Similarly, for segmentation, the deviation in score between seen and unseen data types are computed over different segmentation metric categories, $k \in \{DSC, F2, p, r, H_d\}$ with tolerance, ($tl = 0.05$):
\begin{equation}
    dev\_g = \frac{1}{|k|}\sum_k\begin{cases}
    |(\mathrm{S_k}^{seen}- tl *\mathrm{S_k}^{seen})  - \mathrm{S_k}^{unseen}|, & \text{for } \mathrm{S_k}^{seen} - tl *\mathrm{S_k}^{seen}) \leq  \mathrm{S_k}^{unseen}| \geq \mathrm{S_k}^{seen} + tl *\mathrm{S_k}^{seen}\\
                            0, \quad \text{otherwise.} \\
                         \end{cases}
\end{equation}
%
\subsection*{Challenge setup, and ranking procedure}
% TODO
We set-up challenge website\footnote{https://endocv2021.grand-challenge.org} with an automated docker system for metric-based ranking procedure. Challenge participants were required to perform inference on our cloud-based system that incorporated NVIDIA Tesla V100 GPU and provided test dataset with instructions of using directly on GPU without downloading the data for round 1 and round 2. However, we added an additional round 3 where the challenge participant's trained model were used for inference by the organisers on an an additional unseen sequence dataset. Thus, the challenge consisted of three rounds as summarised below:
\begin{itemize}
    \item Round 1: Test subset-I consisted of: a) 50 samples of each data 1 (unseen modality), data 2 (unseen single sample, C6) and data 3 (mixed center C1-C5 sequence data)
    \item Round 2:  Test subset-II comprised of: a) all 88 samples of each data 1 (unseen modality), 86 samples of data 2 (unseen single sample, C6) and 124 samples of data 3 (mixed C1-C5)
    \item Round 3: Inference on round 3 data was performed by the organisers on the same GPU. This round comprised of: a) 88 samples of each data 1 (unseen modality), 86 samples of data 2 (unseen single sample, C6), 124 samples of data 3 (mixed center C1-C5 sequence data) and an additional set of 420 sequence samples from unseen center C6
\end{itemize}

We conducted elimination for both round 1 and round 2 which was based on the metric scores on the leaderboard and timely submission. In round 2, we eliminated those with very high computational time for inference and metric score consistency. The chosen participants were requested for the method description paper at the EndoCV proceeding~\cite{Ali2021:EndoCVProc} to allow transparent reporting of their methods. All accepted methods were eligible for round 3 evaluation and have been reported in this paper.

Detection ranking was performed as an aggregated score between the average precision and deviation scores between data 3 (seen C1-C5) w.r.t other unseen data in the test set. Similarly, for team ranking on segmentation, we used segmentation metrics and deviation scores for segmentation (between seen and unseen data). Please refer to Section Evaluation metrics for details. An aggregated rank was used to announce winner. In our final ranking reported in this paper, we have additionally used inference time as well. 

==> Introduction.tex <==
% NOTE: DO NOT RESOLVE TRACK CHANGES PLEASE. I HAVE TO THINK AGAIN!!!
\section*{Introduction}
%
Colorectal cancer (CRC) is the third leading cause of cancer deaths, with a reported mortality rate of nearly 51\%~\cite{Bray2018}. CRC can be characterised by early cancer precursors such as adenomas or serrated polyps that may over time lead to cancer. While polypectomy is a standard technique to remove polyps~\cite{kaminski2017increased} by placing a snare (thin wire loop) around the polyp and closing it to cut though the polyp tissue either with diathermy (heat to seal vessels) or without (cold snare polypectomy), identifying small or flat polyps (e.g. lesion less than 10 mm) can be extremely challenging. This is due to complex organ topology of the colon and rectum making the navigation and treatment procedures difficult and requiring expert-level skills.   
% Talk about artifacts and other confusing 
% TODO: add the missed rates (JE)
Similarly, the removal of polyps can very challenging due to constant organ deformations which make it sometimes impossible to keep track of the lesion boundary making the complete resection difficult and subjective to experience of endoscopists. Computer-assisted systems can help to reduce operator subjectivity and enables improved adenoma detection rates (ADR). Thus, computer-aided detection and segmentation methods can assist to localise polyps and guide surgical procedures (e.g. polypectomy) by showing the polyp margins. One of the major requirement of such system is real-time performance and robustness [cite]. 

While machine learning, in particular deep learning, together with tremendous improvements in hardware have enabled the possibility to design networks that can provide real-time performance despite their computational complexity. However, one major challenge in developing these methods is the lack of comprehensive public datasets that can be used for building robust systems. However, in the past decade there has been several attempts made to collect and curate gastrointestinal (GI) datasets that include other GI lesions and polyps. A summary of existing related datasets with polyps are provided in Table~\ref{tab:datasets}. 
%
Kvasir-SEG~\cite{jha2020kvasir} open-access dataset that includes variable resolution single frame images acquired from an Olympus Europe and consists of corresponding annotated polyp masks (and bounding boxes). 
%
The CVC-Clinic research group (Hospital Clinic, Barcelona, Spain) provided three datasets namely, CVC-ColonDB~\cite{bernal2012towards} with 380 images of size 574$\times$500, CVC-ClinicDB~\cite{bernal2015wm} with 612 images of size 384$\times$288 and CVC-VideoClinicDB~\cite{bernal2017miccai} which includes 18 short videos providing 11,954 images of size 384 $\times$ 288. Each dataset provide polyp frames with their corresponding ground truth masks.
%
Similarly, another dataset ETIS-Larib Polyp DB~\cite{silva2014toward} include 196 white light endoscopy frames of size 1224$\times$966 pixels with polyps extracted from 34 sequences with 44 different polyps.
%
The ASU-Mayo polyp database~\cite{tajbakhsh2015automated} (Mayo Clinic in Arizona) includes a total of 30 colonoscopy videos. The dataset is divided into training and testing data. The training dataset consists of 20 videos providing 18,781 frames (i.e. 10 positive videos with polyps and 10 negatives videos without polyps) and 10 videos for testing.
%
The HyperKvasir~\cite{borgli2020hyperkvasir} dataset is another large size dataset but consist of both gastroscopy and colonoscopy examinations and is partly labeled.
%
Kvasir-Capsule~\cite{smedsrud2020kvasir} is a video capsule endoscopy (VCE) data that has 14 different findings including polyps. The data consists of 4,741,504 images collected from 117 videos with 47,238 labelled frames. 
%
A major limitation of the above publicly available datasets is that they consists of either single center or a single population data (i.e. from hospitals of the same country). 
% TODO: include challenge summaries (at max 4-5 lines) here (remove the challenge table)
%

These datasets were also used in colonoscopy challenges. For examples, Kvasir-SEG was used in two challenges in 2020, by "Medico automatic polyp segmentation challenge\footnote{\url{https://multimediaeval.github.io/editions/2020/tasks/medico/}}" , Endotect\footnote{\url{https://endotect.com/}} challenge, and "MedAI: Transparency in Medical Image Segmentation Challenge \footnote{\url{https://www.nora.ai/Competition/image-segmentation.html}}". In 2015, Bernal et al.~\cite{bernal2017comparative} proposed a challenge for an automatic polyp detection and localization from colonoscopy videos using three datasets - CVC-ClinicDB~\cite{bernal2015wm}, ETIS-Larib~\cite{silva2014toward} and the ASU-Mayo polyp database~\cite{tajbakhsh2015automated}. In 2017, Bernal et al. ~\cite{gianadataset2017} proposed the Gastrointestinal Image ANAlysis (GIANA)\footnote{\url{https://endovissub2017-giana.grand-challenge.org/}} sub-challenge aiming to detect and segment polyps from both colonoscopy images and wireless capsule images. In 2018, Bernel et al.~\cite{angermann2017towards,bernal2018polyp}, launched GIANA\footnote{\url{https://giana.grand-challenge.org/}} 2018, where they added the classification task to the challenge to cover the three main tasks related to colonoscopy image analysis: polyp detection, segmentation and classification. 
%
Endoscopic computer vision challenge (EndoCV) launched a multi-center disease detection and segmentation challenge in 2020 (EDD2020~\cite{ali2020endoscopy,ali2021_endoCV2020}) for gastrointestinal lesions that included polyps, dysplasia and cancer. However, this data consisted of only 386 images with only 128 (TODO-check) instances of polyps. 
% TODO: LLL
With the presented EndoCV2021 challenge we release a multicenter dataset that includes five center datasets for training and validation while the test data consisted of four different configurations - a) mixed center data, b) different modality (Narrow-band image modality, NBI & White light image modality,WL), c) hidden sixth center single frame and d) hidden sixth center sequence data.
%
% The dataset is gathered from four different centers with three organ categories: colon, esophagus and stomach. The dataset consists of 386 still image frames acquired from multiple videos.

% This will go at the end (do not remove below)
% While polyp detection and segmentation methods using machine learning, in particular deep learning, have been widely studied and developed, the generalisability of these approaches are not guaranteed. These methods are mostly validated on single center dataset, single modality and uses data acquired from same endoscope. 

% TODO: 
% TODO 1: Summarise the Table 1 dataset and refer to the table
%There exists different gastrointestinal lesion datasets that include images and videos for polyps. Table~\ref{tab:datasets} provides a summary for these datasets showing their target lesions, number of samples and data availability. As shown in the table, Kvasir-SEG~\cite{jha2020kvasir} open-access dataset provides 1000 polyp images and their corresponding ground truth with a varying resolution of $332 \times 487$ to $1920 \times 1072$ pixels. 
%
%The CVC-Clinic research group provide three datasets named, CVC-ColonDB~\cite{bernal2012towards} which includes 380 images of size 574$\times$500, CVC-ClinicDB~\cite{bernal2015wm} which includes 612 images of size 384$\times$288 and CVC-VideoClinicDB~\cite{bernal2017miccai} which includes 18 short videos providing 11,954 images of size 384 $\times$ 288. Each dataset provide polyp frames with their corresponding ground truth. 
%
% The HyperKvasir~\cite{borgli2020hyperkvasir} dataset is collected during gastroscopy and colonoscopy examinations and is partly labeled. This dataset is composed of 110,079 images and 374 videos locating anatomical landmarks, pathological and normal findings.
% %
%
% THIS SEEMS NOT INTERESTING FOR US!
%  The Atlas of GI Endoscope~\cite{{atlas}} contains 1296 of gastrointestinal frames. The El salvador atlas~\cite{gastroatlas} provides a high resolution short videos of gastrointestinal endoscopy including polyps. The data is publicly available online with 5138 video clips with no ground truth. Most of these data are not publicly available online and they require a request from the data provider to have access to it. Additionally, pixel-level annotations are not available in most of them. 
%is a gastrointestinal dataset that includes 23 different findings including anatomical regions, lesions (including polyps, colitis, Barrett’s esophagus) and inflammation (colitis, esophagitis). 
% The data  The dataset provided by

 

%TODO: @NOHA: Summarise this, please remove some challenges that are not popular in community!!! -- We have limited space so focus on high-quality references only
% Some of the previously discussed datasets in Table~\ref{tab:datasets} were used in polyp detection/segmentation challenges. Table~\ref{tab:challenges} summarizes the competition held between 2015 and 2021.  In 2015, Bernal et al.~\cite{bernal2017comparative} proposed a challenge for an automatic polyp detection and localization from colonoscopy videos using CVC-ClinicDB~\cite{bernal2015wm}, ETIS-Larib~\cite{silva2014toward} and the ASU-Mayo polyp database~\cite{tajbakhsh2015automated}. In 2017, Riegler et al.~\cite{riegler2017multimedia} suggested the Medico task\footnote{\url{http://multimediaeval.org/mediaeval2018/medico/}} that requested detection of five different diseases for the gastrointestinal video frames (i.e. including polyps) utilizing the Kvasir dataset~\cite{pogorelov2017kvasir}. In 2017, Bernal et al. ~\cite{gianadataset2017} proposed the Gastrointestinal Image ANAlysis (GIANA)\footnote{\url{https://endovissub2017-giana.grand-challenge.org/}} sub-challenge aiming to detect and segment polyps from both colonoscopy images and wireless capsule images. In 2018, Bernel et al.~\cite{angermann2017towards,bernal2018polyp}, launched GIANA\footnote{\url{https://giana.grand-challenge.org/}} 2018, where they added the classification task to the challenge to cover the three main tasks related to colonoscopy image analysis: polyp detection, segmentation and classification.  Similarly, in 2018, Pogorelov et al.~\cite{pogorelov2018medico} organized a Medico 2018 challenge\footnote{\url{http://multimediaeval.org/mediaeval2018/}} that consisted of a 14,033 GI endoscopy frames from 16 classes. The challenge aimed to develop an efficient method (in terms of MCC and processing speed (FPS)) for GI disease classification. The challenge also focused on the automatic report generation task where they were asked to provide the text report for the provided videos. Similarly, in 2019, hicks et al.~\cite{hicks2020acm} proposed Biomedia challenge, where they proposed the same tasks as Medico 2018~\cite{pogorelov2018medico}. The only difference was the number of videos for the automatic report generation task were increased to 6. Also, the organizer evaluated each method code on their same hardware. In 2019, Ali et al.~\cite{ali2019endoscopy} organized Endoscopic artefact detection challenge(EAD 2019)\footnote{\url{https://ead2019.grand-challenge.org/}} challenge, where they released more than 2192 endoscopic images. The main aim of the challenge was to address key problems in video endoscopy such as multi-class artefact detection, multi-class artefact region segmentation, and  multi-class artefact generalization. In 2020, Ali et al.~\cite{ali2020endoscopy}, proposed endoscopy disease detection and segmentation challenge (EDD)\footnote{\url{https://endocv.grand-challenge.org/}}. Likewise, in 2020, Jha et al.~\cite{jha2020medico} proposed ``Medico automatic polyp segmentation challenge\footnote{\url{https://multimediaeval.github.io/editions/2020/tasks/medico/}}" where they offer automatic polyp segmentation task and efficiency task. The challenge used Kvasir-SEG~\cite{jha2020kvasir} dataset as the training dataset and provided a new test set that consisted of 160 polyp images for evaluation of the methods. Similarly, in 2020, hicks et al.\cite{hicks2021endotect} proposed endotect\footnote{\url{https://endotect.com/}} challenge,  where they propose automatic GI tract classification task on 23 different classes of GI findings dataset and binary polyp segmentation task using HyperKvasir~\cite{borgli2020hyperkvasir} dataset. The organizer released 721 new GI findings for classification task and 200 new polyps for segmentation task as the test dataset. 

%In the recent years, there is a rise of competitions and challenges for benchmarking the machine learning algorithms. However, there is still need for such competitions and challenges for comprehensive benchmarking of the algorithm on the GI endoscopy dataset especially because of nature of endoscopic findings, variation in procedure, device and protocols~\cite{jha2021comprehensive}. The major limitation in the current challenges are most of competitions are organized on limited  single organ data dataset. Also, the some of the current competitions hide the dataset or requires prior consenting before using such dataset. Additionally, most of the above challenge use same training dataset or extend the challenge by adding more number of samples to the training dataset. They mostly release new new test dataset for evaluating competitions. However, it can be subjected to bias as some of the participants may have been using these dataset and have prior idea about the algorithms that might work. 

%Motivated by success of the previous challenge, we initiate collaboration with six research institution and hospitals From UK, Norway, Egypt, France, and Italy and have collected, curated, and annotated new dataset specifically for our competition.  By doing these, we provide the community with the new dataset and also provide the same time frame to work on the same dataset. Moreover, we release the dataset and make it fully open-access so that it does not require any consenting. 

% @Noha/Debesh: Please check which CVC-ColonDB was used in challenge? if only CVC-CLinicDB then please check if they have same sample size or different?
\begin{table*}[t!]
% 	\def\arraystretch{1.2}
	\centering
	\footnotesize
% Study type: Multi  or single ? @Debesh TODO
	\begin{tabular}{l|c|c|c|c|c|c|c} 
		\hline
% 		ADD: Resolution, Type of polyps, # of patients 
		\bf Dataset &\bf Findings & \bf \# of samples & \bf Resolution & \bf Modality & \bf Study type & \bf Challenge & \bf Availability \\ \hline
		%CVC-356~\cite{bernal2017miccai} & Polyps & 356 images$^\dag$&  by request$^\bullet$ \\ \hline
		
		Kvasir-SEG~\cite{jha2020kvasir} & Polyps & 1000 images$^\dag$& \begin{tabular}[t]{@{}l@{}} 332$\times$487 - \\ 1920$\times$1072\end{tabular}&WL  &Single &\shortstack{Medico\\ \& MedAI} & open academic  \\ \hline
		
		CVC-ColonDB~\cite{bernal2012towards}& Polyps & 380 images$^\dag$ $^\dagger$  &WL $574\times500$ &WL  &Single & APD2015 & by request$^\bullet$ \\ 
		\hline
				
		CVC-ClinicDB~\cite{bernal2015wm} & Polyps & 612 images$^\dag$& 384$\times$288  &WL &Single &APD2015 & open academic \\ \hline 
		
		CVC-VideoClinicDB~\cite{bernal2017miccai} & Polyps & 11,954 images$^\dag$ & 384$\times$288 &- &Single  &APD2015 & by request$^\bullet$ \\ \hline
		
		ETIS-Larib Polyp DB~\cite{silva2014toward} & Polyps & 196 images$^\dag$  &1224$\times$966 & WLE &Single  & APD2015 &open academic \\ \hline
		
		\begin{tabular}[t]{@{}l@{}} ASU-Mayo polyp  \\ database~\cite{tajbakhsh2015automated}\end{tabular}  & Polyps & 18,781 images$^\dag$ &$688\times 550$   &  &Single  & APD2015&by request$^\bullet$  \\ \hline
		
		HyperKvasir~\cite{borgli2020hyperkvasir} & \begin{tabular}[t]{@{}l@{}} GI findings \\ with polyps\end{tabular} & \begin{tabular}[t]{@{}l@{}} 110,079 images \\ \& 374 videos\end{tabular} &\shortstack{$720\times 576$\\to $1920\times 1072$}  & WLE &Single & NA & open academic \\ \hline
		
		Kvasir-Capsule~\cite{smedsrud2020kvasir} & \begin{tabular}[t]{@{}l@{}} GI findings \\ with polyps$^\diamond$\end{tabular} & 4,741,504 images & \shortstack{$256 \times 256$\\ to $512 \times512$}  &  VCE & Single & NA & open academic \\ \hline
		
		
	    EDD2020~\cite{ali2020endoscopy,ali2021_endoCV2020} & \begin{tabular}[t]{@{}l@{}} GI findings \\ with polyps\end{tabular} & 386 images  & & \begin{tabular}[t]{@{}l@{}}WLE,\\ NBI\end{tabular} & Multi & EndoCV2020 & open academic\\ \hline %(2342$^\sharp$, 597$^\ast$, 2199$\Delta$ $^\dag)

		PolypGen~\cite{ali2021polypgen}& \begin{tabular}[t]{@{}l@{}} Polyp & \\non-polyp \end{tabular} &  \begin{tabular}[t]{@{}l@{}} \shortstack{3446 images \\ including \\sequence data$^\dag$}\end{tabular} & \shortstack{$384\times288$\\ to $1920\times1080$} &\begin{tabular}[t]{@{}l@{}} WLE, \\NBI\\ (test)\end{tabular} & Multi & EndoCV2021 & open academic \\ \hline
	   \multicolumn{6}{l}{$^\dag$Including ground truth segmentation masks \hspace{.1cm}
	   $^\ddagger$Contour \hspace{.1cm}
	   $^\diamond$Video capsule endoscopy\hspace{.1cm}
	   $^\bullet$Not available anymore}\\
	    \multicolumn{4}{l}{$^\clubsuit$Medical atlas for education with several low-quality samples of various GI findings, \hspace{.1cm}}\\
	   %$^\theta$ Released  as test data} \\ % This is minor 
	 \end{tabular}
     \caption{An overview of existing gastrointestinal lesion datasets including polyps}  
	\label{tab:datasets}
\end{table*}

%         %https://polyp.grand-challenge.org/site/polyp/asumayo/
% 		KID~\cite{koulaouzidis2017kid} & \begin{tabular}[c]{@{}l@{}}Angiectasia,\\ bleeding,\\ inflammations$^\diamond$
%  \end{tabular} & \begin{tabular}[c]{@{}l@{}}2371 images,\\ 47 videos \end{tabular}   & & &  & open academic$^\bullet$\\ \hline
	   %Atlas of GI Endoscope~\cite{{atlas}}& GI lesions & 1295 images &240$\times$352  & & & unknown$^\bullet$ \\   \hline
	   %El salvador atlas~\cite{gastroatlas} & GI lesions &  5071 video clips & 240$\times$352 &  & & open academic$^\clubsuit$ \\ \hline

% Not needed (contracted in Table 1)
% \begin{table*}[t!]
% \centering
% \begin{tabular}{l|c|c|c} 
% \hline
% \bf Challenge Name &\bf Year & \bf Dataset Used & \bf Availability \\ \hline

% \shortstack{Automatic Polyp Detection in Colonoscopy videos 2015~\cite{bernal2017comparative}}  &2015 &\shortstack{CVC-ClinicDB,\\ ETIS-Larib,\\\shortstack{ASU-Mayo Clinic\\ Colonoscopy Video (c)\\ Database }}, &By request \\ \hline

% \text{Medico task} 2017~\cite{riegler2017multimedia}  &2017 &Kvasir & Open-access \\ \hline


% GIANA 2017~\cite{gianadataset2017} &2017 &CVC-ClinicDB &by request \\ \hline

% GIANA 2018~\cite{angermann2017towards,bernal2018polyp}  &2018 &CVC-ClinicDB &by request\\ \hline

% Medico task 2018~\cite{pogorelov2018medico} &2018 &Kvasir &open-access  \\  \hline

% EAD 2019~\cite{ali2019endoscopy}  & 2019 & &open-access  \\   \hline

% BioMedia grand challenge 2019~\cite{hicks2019acm}  &2019 &Kvasir &open-access  \\  \hline

% EAD 2020~\cite{ali2019endoscopy} &2020 & &open-access  \\  \hline

% EDD 2020~\cite{ali2020endoscopy} &2020 & & open-access \\ \hline

% \shortstack{Medico Automatic polyp segmentation challenge~\cite{jha2020medico}} &2020 &Kvasir-SEG &open-access  \\ \hline

% Endotect Challenge~\cite{hicks2020endotect} &2020 &Kvasir-SEG &open-access  \\ \hline


% EndoCV2021 Challenge (Ours) &2021 & PolypGen & open-access \\ \hline 

% 	 \end{tabular}
%      \caption{Overview of GI endoscopy challenges}  
% 	\label{tab:challenges}
% \end{table*}

==> Particiapant_Algo_submissionHandlingg.tex <==
\subsection*{Participants, algorithms and submission handling}
\begin{itemize}
    \item Summarize in words regarding numbers and leaderboard and methods (Felix)
    \item Summary table (Sharib will do this)
    \item Link all to Suppl. Material 2 (Sharib)
    \begin{itemize}
        \item Leader board
        \item Algorithms in detail
        \item Suppl. Note
        \item Executable versions if available (Ask for links for entries with yes!, not mandatory)
    \end{itemize}
\end{itemize}


==> Quantitative_performance_criteria.tex <==
\section*{EndoCV challenge quantitative evaluation criteria}
\begin{itemize}
    \item Suppl. Table with all the links
    \item Table with parameters configuration for each team
\end{itemize}


==> RelatedWork.tex <==
%
%
\section*{Related work}
In this section, we briefly describe related works on detection, localisation and segmentation. 
\subsection*{Detection and localisation}
While classification methods are frame-based classifiers for polyps~\cite{tajbakhsh2015automatic, park2016colonoscopic, ribeiro2016colonic}, detection methods provide both classification and localisation of polyps~\cite{2019Polyp,urban2018deep} which can direct clinicians to the site of interest, and can be additionally used for counting polyps to assess disease burden in patients. With the advancements of object detection architectures, recent methods are end-to-end networks providing better detection performance and improved speed. The state-of-the-art methods are broadly divided into two categories: multi-stage detectors and single-stage detectors. The multi-stage detector methods include Regional-Based Convolutional Neural Network (R-CNN)~\cite{girshick2014rich}, Fast R-CNN~\cite{girshick2015fast}, Faster R-CNN~\cite{ren2015faster}, Region-based fully convolutional networks (R-FCN)~\cite{dai2016r}, Feature Pyramid Network (FPN)~\cite{lin2017feature} and Cascade R-CNN~\cite{cai2018cascade}. On the other hand, the One-stage detectors directly provide the predicted output (bounding boxes and object classification) from input images without the region of interest (ROI) proposal stage. The One-stage detector methods include Single-Shot Multibox Detector (SSD)~\cite{liu2016ssd}, Yolo~\cite{redmon2016you}, RetinaNet~\cite{lin2017focal} and Efficientdet~\cite{tan2020efficientdet}.  

Different studies have been conducted in the literature that focused on polyp detection by employing both multi-stage detectors and single-stage detectors. \textbf{Multi-stage Detectors:} Shin et al. \cite{younghak2017} used a transfer learning strategy based on Faster R-CNN architecture with the Inception ResNet backbone to detect polyps. Qadir et al. \cite{2019Polyp} adapted Mask R-CNN~\cite{he2017mask} to detect colorectal polyps and evaluate its performance with different CNN including ResNet50~\cite{he2016deep}, ResNet101~\cite{he2016deep} and Inception ResNetV2~\cite{2016Inception} as its feature extractor. Despite the speed limitation, multi-stage detectors are widely used in the detection task of endoscopy data science challenges due to their competitive performance on evaluation metrics. \textbf{Single-stage Detectors:} Urban et al.~\cite{urban2018deep} used YOLO to detect polyps in real-time, which also resulted in high detection performance. Lee et al.~\cite{lee2020real} employed YOLOv2~\cite{redmon2017yolo9000} and validated the proposed approach on four independent dataset. They reported a real-time performance and high sensitivity and specificity on all datasets. Zhang et al.~\cite{zhang2018polyp} proposed the ResYOLO network that adds residual learning modules into the YOLO architecture to train deeper networks. They reported a near-real-time performance for the ResYOLO network depending on the hardware used. Zhang et al.~\cite{zhang2019real} proposed an enhanced SSD named SSD for Gastric Polyps (SSD-GPNet) for real-time gastric polyp detection. SSD-GPNet concatenates feature maps from lower layers and deconvolves higher layers using different pooling techniques. Additionally, Jha et al.~\cite{} performed an extensive study where they compared the performance of both single stage and multi-stage detectors with different backbones. YOLOv3~\cite{redmon2018yolov3} with darknet53 backbone and YOLOv4 showed IOU and average precision (AP) over 0.80\%  and real-time FPS over 45. Moreover, there exist methods the relied on \textbf{Anchor-free detectors} to locate the polyps where they claim to detect polyps without the definition of anchors such as CornerNet~\cite{law2018cornernet} and ExtremeNet~\cite{zhou2019bottom}. Zhou et al.~\cite{2019Objects} proposed the CenterNet, which treats each object as a point and increases the speed significantly while ensuring the accuracy is acceptable. While Wang et al.~\cite{wang2019afp} achieved state-of-the-art results on automatic polyp detection in real-time situations using anchor-free object detection methods. In addition to these works, Multi-stage, Single-stage and other types of detectors have been widely used by participants teams in different polyp detection datasets and challenges such as MICCAI'15~\cite{7840040}, ROBUST-MIS~\cite{ross2020robust}, EAD2019~\cite{ali2019endoscopy} and EndoCV2020~\cite{ali2021deep}.


\subsection*{Segmentation}
Semantic segmentation is the process of grouping related pixels in an image to an object of the same category. Deep learning has been very successful in the field of the medical domain, convolutional neural networks (CNN) based techniques were suggested to generate complete and precise segmentation outputs without requiring any post-processing. In deep learning, medical segmentation methods can be categorized into four categories: Models based on fully convolutional networks, Models based on Encoder-Decoder architecture, Models based on Pyramid-based architecture and Models based on Dilated Convolution Architecture.

%In the literature,
\textbf{Models based on fully convolutional networks:
} Brandao et al. \cite{brandao2017fully} proposed three different FCN-based architectures for detection and segmentation of polyps from colonoscopy images. Zhang et al.  \cite{zhang2017automated} proposed multi-step practice for the polyp segmentation. The former step includes region proposal generation using FCN, and the latter step uses spatial features and a random forest classifier for the refinement process. A similar method was introduced by Akbari et al. \cite{akbari2018polyp} which uses patch selection while training FCN and Otsu thresholding to find the accurate location of polyp. Guo et al. \cite{guo2019giana} describe two methods based on FCN for Gastrointestinal ImageANALysis-(GIANA) polyp segmentation sub-challenge. 

\textbf{Models based on Encoder-Decoder architecture:} Nguyen and Slee \cite{nguyen2019robust} proposed multiple deep encoder-decoder networks to capture multi-level contextual information and learn rich features during training. Zhou et al.~\cite{zhou2018unet++} proposed UNet++, a deeply-supervised encoder-decoder network that showed good results on polyp segmentation task.  Similarly,  Jha et. al~\cite{jha2019resunet++} proposed ResUNet++ that combines series of residual block, squeeze and excitation network, atrous spatial pyramid pooling, and attention block.  The architecture was designed specially for polyp segmentation. Afterward, Jha et al.~\cite{jha2020doubleu} proposed a general medical image segmentation architecture namely, DoubleU-Net, which stacks two U-Net inseparable of each other. Likewise, Tomar et al.~\cite{tomar2021ddanet} proposed dual-decoder attention network (DDANet) that utilizes residual learning and the squeeze and excitation network. Srivastava et al.~\cite{srivastava2021msrf} proposed Multi-Scale Residual Fusion Network (MSRF-Net) which is based on DSDF  block. The DSDF block comprises  of  residual  dense  connections that allows information exchange across multiple scales. Tomar et al.~\cite{tomar2021fanet} proposed a feedback attention network (FANet) that uses iterative mechanism to refine the prediction of biomedical images. The architure showed improved results over seven biomedical datasets.  Similarly, Mahmud et al.~\cite{mahmud2021polypsegnet} integrated dilated inception blocks into each unit layer and aggregate the features of the different receptive fields to capture better-generalized feature representations. Huang et al.~\cite{huang2021hardnet} proposed a low memory traffic, fast and accurate method for the polyp segmentation achieving 86 frames per second (FPS). Later, Zhang et al.~\cite{zhang2021transfuse} proposed a hybrid method combining both transformer-based network and CNN to capture global dependencies and the low-level spatial features for the segmentation task. Most encoder-decoder architectures were evaluated only on still images. Ji et al.~\cite{ji2021progressively} proposed a Progressively Normalized Self-Attention Network (PNS-Net) that was designed for video polyp segmentation. The framework compromises of normalized self attention block followed by progressive learning strategy.   

\textbf{Models based on Pyramid-based architecture:} Jia et al. \cite{Jia2020} proposed a pyramid-based model named Polyp Net (PLPNet) for automated pixel-level polyp classification in colonoscopy images. Also, Guo et al. \cite{Guo2019} employed the Pyramid Scene Parsing Network (PSPNet) \cite{Zhao2017} with SegNet \cite{badrinarayanan2017segnet} and U-Net \cite{ronneberger2015u} as an ensemble deep learning model. The proposed model achieved a range of improvement of 1.98\%–6.38\% compared with a single basic trainer.


\textbf{Models based on Dilated Convolution Architecture:} In \cite{sun2019colorectal} the dilated convolution was used in the last block of the encoder while in \cite{safarov2021denseunet} it is used in all encoder blocks. Though \cite{safarov2021denseunet} used a mesh of attention blocks and residual block as a decoder. Both methods  \cite{sun2019colorectal,safarov2021denseunet} tested there model on CVC-ClinicDB achieving F1-score of 96.106 and 96.043, respectively. Furthermore, Nested Dilation Network (NDN) \cite{wang2019nested} has been designed to segment lesions and have been tested on the GIANA2018 dataset. The proposed model achieved a range of improvements of Dice = [1.79\%-3.01\%] compared to \cite{nguyen2018colorectal}, and \cite{wickstrom2018uncertainty}, respectively.

%



%\section*{Related work}
%\subsection*{Detection and localisation}

% Before directly jumping into the single-stage, multi-stage networks vs., I think it is better to write some sentences that mention the very early work that uses CNNs

%While classification methods are frame-based classifiers for polyps~\cite{tajbakhsh2015automatic, park2016colonoscopic, ribeiro2016colonic}, detection methods provide both classification and localisation of polyps~\cite{2019Polyp,urban2018deep} which can direct clinicians to the site of interest, and can be additionally used for counting polyps to assess disease burden in patients. With the advancements of object detection architectures, recent methods are end-to-end networks providing better detection performance and improved speed. The state-of-the-art methods are broadly divided into two categories: multi-stage detectors and single-stage detectors. In this section, we provide the evolution of these methods with their application in polyp detection. 
%
%\paragraph{Multi-stage detectors}
% Automatic Colon Polyp Detection Using Region Based Deep CNN and Post Learning Approaches, Shin et al => Faster RCNN SPP-Net \cite{he2015spatial},
% Abnormal Colon Polyp Image Synthesis Using Conditional Adversarial Networks for Improved Detection Performance, shin et al => GAN for augmenting, Faster RCNN for detection
% Development of a real-time endoscopic image diagnosis support system using deep learning technology in colonoscopy, Yamada et al. => Faster RCNN
%The multi-stage object detectors first find the region-of-interest where the objects may exist, then fine-tune the boundary of the candidate region and predict the category of the objects.
%Faster R-CNN~\cite{ren2015faster} designed a region proposal network (RPN) to replace the selective search algorithm of previous R-CNN~\cite{girshick2014rich} and Fast R-CNN \cite{girshick2015fast} approaches, realizing the first end-to-end trainable object detection method with improved performance and speed compared to former methods. Different extensions have been made to the Faster R-CNN to achieve an improved performance, where, Cai et al.\cite{cai2018cascade} proposed the Cascade R-CNN which handles the overfitting and inference mismatch between bounding boxes cause by Faster R-CNN. Moreover, He et al.~\cite{he2017mask} extended the Faster R-CNN by using the feature pyramid networks (FPN) to provide instance detection and segmentation well-known as Mask R-CNN. Even though the multi-stage detectors have shown improved performance but its application has been limited due to its inability for achieving real-time performance.

%In the field of colorectal polyp detection, Shin et al. \cite{younghak2017} used transfer learning strategy based on Faster R-CNN architecture with the Inception ResNet backbone to detect polyps. Qadir et al. \cite{2019Polyp} adapted Mask R-CNN to detect colorectal polyps and evaluate its performance with different CNN including ResNet50 \cite{he2016deep}, ResNet101 \cite{he2016deep} and Inception ResNetV2 \cite{2016Inception} as its feature extractor. Despite the speed limitation, the multi-stage detectors are widely used in the detection task of endoscopy data science challenges due to its competitive performance on evaluation metrics. *
% 

% In the field of colorectal polyp detection, Shin et al. \cite{younghak2017} used transfer learning strategy based on Faster R-CNN architecture with the Inception ResNet backbone to detect polyps. The proposed method got a superior detection performance in terms of precision and recall. But the detection processing time in each frame is not suit for real-time application. Qadir et al. \cite{2019Polyp} adapt Mask R-CNN to detect colorectal polyps and evaluate its performance with different CNN including ResNet50 \cite{he2016deep}, ResNet101 \cite{he2016deep} and Inception ResNet v2 \cite{2016Inception} as its feature extractor. Despite the speed limitation, the multi-stage detectors are widely used for challenges due to its better performance. The Faster R-CNN, Cascade R-CNN \cite{cai2018cascade} and Mask R-CNN were very popular among the top teams in EAD2019, EAD2020 and EDD2020.

%\paragraph{Single-stage detectors}


%Real-time detection of polyps during the colonoscopy procedure is crucial for its clinical usability; therefore, fast processing of the video frames is a high priority factor when selecting the object detection architecture. The single-stage detectors enhance the speed of two-stage detectors performance by merging the region proposal slayer with the classification layer. Different single-stage frameworks are available in the literature such as Single Shot MultiBox Detector (SSD) \cite{liu2016ssd} and YOLO \cite{redmon2016you}


%Several studies employed single-stage detectors due to their superior speed compared to other detectors. Urban et al. \cite{urban2018deep} used YOLO to detect polyps in real-time, which also resulted in high detection performance. Lee et al. \cite{lee2020real} employed YOLOv2 \cite{redmon2017yolo9000} and validated the proposed approach on four independent dataset. They reported a real-time performance and high sensitivity and specificity on all datasets. Zhang et al. \cite{zhang2018polyp} proposed the ResYOLO network that adds residual learning modules into the YOLO architecture to train deeper networks. They reported a near-real-time performance for the ResYOLO network depending on the hardware used. Zhang et al. \cite{zhang2019real} proposed an enhanced SSD named SSD for Gastric Polyps (SSD-GPNet) for real-time gastric polyp detection. SSD-GPNet concatenates feature maps from lower layers and deconvolved higher layers using different pooling techniques.


%\paragraph{Other detectors}
%\paragraph{Anchor-free detectors}
% Change the paragraph name from 'Anchor-free detectors' to 'other detectors'
%One of the newly emerging types of object detection methods is anchor-free detectors. The single-stage and multi-stage detectors are based on predefined anchors, which have many drawbacks. For example, the performance of the detectors depends on the number, size and aspect ratio of the preset anchors. In addition, the preset anchors are aimed at the specific dataset, which may not have good generalizability. Therefore, the anchor-free detectors claim to detect objects without the definition of anchors. CornerNet \cite{law2018cornernet} uses corner pooling to generate heatmap, embedding vector, and coordinate offset. The heatmap is responsible for judging whether a point is the corner point of an object, and the embedding vector is used to judge whether the two corner points are the upper left corner and the lower right corner belong to the same object. The coordinate offset is used to refine the coordinate position. The idea of ExtremeNet \cite{zhou2019bottom} is similar and it predicts five points including the center point and four vertices. Duan et al. \cite{duan2019centernet} further consider the center point information of the object based on the CornerNet to reduce the false positive rate. Zhou et al. \cite{2019Objects} proposed the CenterNet, which treats each object as a point and increases the speed significantly while ensuring the accuracy is acceptable.

%Because of the real-time requirements of polyp detection methods during the colonoscopy in the clinical practice, the anchor-free detectors have received more and more attention. Wang et al. \cite{wang2019afp} achieved state-of-the-art results on automatic polyp detection in real-time situation using anchor-free object detection methods.

%Furthermore, Transformer-based detector is another type of object detector. Compared with CNN, the transformer based on the attention mechanism can better utilize the global information of the image. Transformer has achieved surpassing results compared to the state-of-the-art on different vision tasks. Detection Transformer (DETR) \cite{2020End} and Deformable DETR \cite{2020Deformable} are two representative vision transformers for object detection. Although there is no transformer-based detector for polyp detection currently, this is a direction worth exploring.

%Multi-stage, Single-stage and other types of detectors have been widely used by participants teams in different polyp detection datasets and challenges such as MICCAI'15 \cite{7840040}, ROBUST-MIS~\cite{ross2020robust}, EAD2019~\cite{ali2019endoscopy} and EndoCV2020~\cite{ali2021deep}.

%\subsection*{Segmentation}
%Semantic segmentation is the processes of grouping related pixels in an image to an object of the same category. Deep learning has been very successfully in the field of the medical domain, convolutional neural networks (CNN) based techniques were suggested to generate complete and precise segmentation outputs without requiring any post-processing. In deep learning, medical segmentation methods can be categorized into four categories: Models based on fully convolutional networks, Models based on Encoder-Decoder architecture, Models based on Pyramid-based architecture and Models based on Dilated Convolution Architecture.

%\paragraph{Models based on fully convolutional networks} 
%Brandao et al. \cite{brandao2017fully} proposed three different FCN-based architectures for detection and segmentation of polyps from colonoscopy images. Zhang et al.  \cite{zhang2017automated} proposed multi-step practice for the polyp segmentation. The former step includes region proposal generation using FCN, and the latter step uses spatial features and a random forest classifier for the refinement process. A similar method was introduced by Akbari et al. \cite{akbari2018polyp} which uses patch selection while training FCN and Otsu thresholding to find the accurate location of polyp. Guo et al. \cite{guo2019giana} describe two methods based on FCN for Gastrointestinal ImageANALysis-(GIANA) polyp segmentation sub-challenge. The same group evaluated and validated their proposed approach Dilated ResFCN on the same dataset \cite{guo2020polyp}.

%\paragraph{Models based on Encoder-Decoder architecture} 
%An encoder-decoder-based U-Net \cite{ronneberger2015u} architecture was primarily designed for the biomedical image segmentation task. Recently, many variants of U-Net based models have been proposed for several segmentation tasks such as lungs segmentation \cite{fan2020inf,oulefki2021automatic}, liver tumor segmentation \cite{li2015automatic}, cell segmentation \cite{akram2016cell} and so on. \parFor the polyp segmentation task, Nguyen and Slee \cite{nguyen2019robust} proposed multiple deep encoder-decoder networks to capture multi-level contextual information and learn rich features during training. A similar method was by Debesh et. al \cite{jha2020doubleu} introduced the DoubleU-Net  which stacks two U-Net inseparable of each other. In order to overcome the limitation of traditional U-Net and boost the learning feature representation of the network, UNet++ \cite{zhou2019unet++} proposed redesigned skip-connection approach with the integration of multi-scale semantic features. Similarly, Mahmud et al. \cite{mahmud2021polypsegnet} integrated dilated inception blocks into each unit layer and aggregate the features of the different receptive fields to capture better-generalized feature representations. In past years, attention-based techniques have been widely explored in the medical domain due to its capability of integrating local and global features efficiently \cite{nie2018asdnet,jin2020ra}. In \cite{fan2020pranet}, a parallel reverse attention network (PraNet) was proposed for the accurate segmentation of polyp in colonoscopy images. Further, a multi-scale attention-based network was proposed to enhance the segmentation performance by restricting unessential features \cite{poudel2021deep}. Huang et al. \cite{huang2021hardnet} proposed a low memory traffic, fast and accurate method for the polyp segmentation achieving 86 frames per second (FPS). Later, Zhang et al. \cite{zhang2021transfuse} proposed a hybrid method combining both transformer-based network and CNN to capture global dependencies and the low-level spatial features for the segmentation task.

%Recently, a Transformer-based network has been employed for the segmentation task.


%\paragraph{Models based on Pyramid-based architecture}
%An image pyramid, hierarchy, or multi-resolution is a technique that successively resizes the image in order to extract features with different scales \cite{burger2016digital}. The core principle of the pyramid technique has traditionally been employed in various image processing applications. Naturally, this technique has been imposed in designing deep learning architectures to make them multi-resolution invariant, thereby enhancing overall performance. Pyramid Scene Parsing Network (PSPNet) \cite{Zhao2017}, and Feature Pyramid Network (FPN) \cite{Li2019} are two successful examples of pyramid-based deep learning models for segmentation tasks.

%Although pyramid-based models have been employed frequently in the literature, only a few published works have used them in the polyp segmentation domain. Jia et al. \cite{Jia2020} proposed Polyp Net (PLPNet) for automated pixel-level polyp classification in colonoscopy images. The proposed model consists mainly of 4 components, namely ResNet50 \cite{He2016}, 4-stages FPN \cite{Li2019}, Region Proposal \& ROI \cite{Ren2017a}, and FCN \cite{long2015fully}, respectively. First, the model is trained using only the first three components to properly adjust the network's weights, then the entire model's weights are frozen to train the last stage (i.e., FCN), thereby generating the masks. The proposed model performed remarkably well on CVC-612. In Guo et al. \cite{Guo2019}, PSPNet employed with SegNet \cite{badrinarayanan2017segnet} and U-Net \cite{ronneberger2015u} as an ensemble deep learning model. A voting scheme was used to produce the segmentation masks. The performance of this model was evaluated using both intersections over union IoU and Dice similarity on three databases, namely, cvc300, CVC-ClinicDB, and ETIS. The proposed model achieved a range of improvement of 1.98\%–6.38\% compared with a single basic trainer \cite{Guo2019}.

%\paragraph{Models based on Dilated Convolution Architecture}
%Dilated convolution or in other term (atrous convolution) refers to the normal convolution process with a defined spatial gap between the kernel's weights. Dilated convolution enable the convolution process to expand the  of the receptive field without loss of resolution or coverage \cite{chen2017deeplab}, hence, capturing the global context.Dilated convolution have been imposed in various models such as UNet-based models \cite{sun2019colorectal,safarov2021denseunet} and Deeplab-based models \cite{xiao2018semantic,nguyen2020contour} to enhance the polyp segmentation accuracy. 

%In \cite{sun2019colorectal} the dilated convolution was used in the last block of the encoder while in \cite{safarov2021denseunet} it is used in all encoder blocks. Though the later used a mesh of attention blocks and residual block as a decoder. Both proposed works \cite{sun2019colorectal,safarov2021denseunet} were tested on CVC-ClinicDB achieving F1-score of 96.106 and 96.043, respectively. However, different test splits were used in both methods therefore direct comparison between them is not valid. 

%Both proposed work in \cite{xiao2018semantic,nguyen2020contour} used DeeplabV3 \cite{chen2017deeplab} as a backbone. The essence of DeeplabV3 \cite{chen2017deeplab} is the usage of atrous spatial pyramid pooling which combines dilated convolution with spatial pyramid pooling. Though in \cite{xiao2018semantic}, Long Short-Term Memory (LSTM) \cite{hochreiter1997long} was added to retain the location information of polyps from DeepLabV3 while \cite{nguyen2020contour} used an ensemble of DeeplabV3+ \cite{chen2018encoder} applied to multiple image scales. As a complementary strategy for improving a model's segmentation capability, \cite{chen2018encoder} proposed a boundary-aware data augmentation method in which a random circle region is selected randomly and sets it's pixels values arbitrary.  

%Nested Dilation Network (NDN) have been designed to segment lesions \cite{wang2019nested}. The core principle of the proposed model is the usage of residual nested dilated convolution blocks (RnD blocks) to enhance the model's capability to identify targets of various sizes \cite{wang2019nested}. The proposed model evaluated on five sub-tasks from Medical Segmentation Decathlon challenge and GIANA2018 challenge. On the polyp segmentation task (GIANA2018), the proposed model achieved a range of improvements of Dice=[1.79\%-3.01\%] compared to \cite{nguyen2018colorectal}, and \cite{wickstrom2018uncertainty}, respectively.



==> Results.tex <==
%
\section*{Results}
%
%
\subsubsection*{On 100\% test data}
%
\subsection*{Qualitative results}
%
\subsection*{Clinical applicability quantification}
%
\subsection*{Statistical analysis}





==> TheEndoCV_challenge.tex <==
%
\section*{The EndoCV challenge: Dataset, Evaluation and method submissions}
%
% Page info: To be written by organisers, please consult before making any changes here!
%%%
\subsection*{Datasets}
%%
%TODO: put sample images
%

%
%
\begin{figure}[t!]
    \centering
    \includegraphics[width= 1.0\textwidth]{Figures/fig1/train_test_genCounts_EAD_EDD2020.jpg}
    \caption{\textbf{Dataset for EndoCV2020}: Train and test annotations for sub-challenge on artefact (A,B) and disease (C) detection and segmentation for each class label.}
    \label{fig:dataset_samples}
\end{figure}
%
\subsubsection*{Endoscopy Artefact Detection and Segmentation (EAD2020)}
%
% Sample images for artefact detection
%
Training and test dataset both represent endoscopy video frames from varied human organs. Training cases have annotated multi-class artefacts present in that frame. A similar proportion of the testing dataset annotated with multi-class artefacts in each frame except the frames exclusive of training data. Endoscopy videos sequences were also provided such that the one sequential segment will have ground truth labels that can be used for training while the other segment will be used only for testing (no ground truth released). For generalisation, only test frames and video sequences were provided from an unseen institution (data not present in either detection or segmentation task categories). 

% TODO: contract them ---> Make in a table
% TODO: put teams per task  and submissions
\begin{table}[t!]
\centering
\begin{tabular}{l|l|c|c|c|c|c}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{EndoCV}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Tasks}}}& \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\# of classes}}} & \multicolumn{2}{c}{\textbf{\# of frames}} & \multicolumn{2}{|c}{\textbf{\# of annotations}} \\ \cline{4-7} 
%
\multicolumn{1}{c|}{} & \multicolumn{1}{|c}{} &\multicolumn{1}{|c}{} &\multicolumn{1}{|c}{\textbf{Train}}  & \textbf{Test}& \textbf{Train}          & \textbf{Test}         \\ \hline
%
\multirow{3}{*}{EAD2020}& Detection task & 8 & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}single: 2299\\ seq.: 233\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}single: 237\\ seq.: 80\end{tabular}} & 31069                   & 7750                  \\ \cline{2-7} 
& Segmentation task & 5  & 573  & 162  & 3248 & 398\\ \cline{2-7} 
& Generalisation task & 8  & na & 99 & na  & 3013 \\ \hline
\multirow{2}{*}{EDD2020} & Detection task & 5 & 386 & 43 & 749 & 68 \\ \cline{2-7} 
& Segmentation task & 5 & 386 & 43 & 749 & 68 \\ \hline
\end{tabular}
\end{table}
%
% Train dataset:
% a) Detection task: 2200 single frame data from 20 videos and 5 frame sequences with 331 frames from another 5 GI tract endoscopy videos
% b) Semantic segmentation task: 573 single frame data which was a sub-set of detection task data collected from 20 videos
% Test dataset:
% a) Detection task:
% i) Single frame: 237 single frames were used from 20 videos 
% ii) sequence frames: Two short sequences from two different patient videos with in total of 80 frames
% b) Semantic segmentation task: 162 frames were released which consisted of the subset single frames from detection test data
% c) out-of-sample generalisation task: 99 frames 

\subsubsection*{Endoscopy Disease Detection and Segmentation (EDD2020)}
%
% Sample images for disease detection
%
%

\subsubsection*{Annotation protocol}
%%
A team of two clinical experts determined the class labels for artefact detection challenge while for disease detection challenge we consulted with four clinical experts regarding the class labels in the GI tract endoscopy. For each sub-challenge at least two clinical experts sampled the video frames from a small sub-set of video data. These frames were then taken as reference to produce bounding box annotations for the remaining train-test dataset by 4 experienced postdoctoral fellows. Finally, further validation by 3 local experts (clinical endoscopists) was carried out to assure the reference standard. The ground-truth labels were
randomly sampled (1 per 20 frames) during this process. However, after the completion of this phase the entire annotation was
discussed and reviewed together.
% Annotation Protocols:
%
Following annotation strategies were used by both clinical experts and researchers:
\begin{itemize}
    \item  For the same region, multiple boxes (for detection) or pixel-wise delineation (for semantic segmentation) were performed if the region belonged to more than 1 class (see Fig. XX)
    \item The minimal box sizes were used to describe the class region and similarly possible small annotation areas for semantic segmentation were merged instead of having multiple small boxes/regions
    \item Each class type was determined to be distinctive and general across all datasets
\end{itemize}

\subsection*{Evaluation metrics}

The challenge problems fall into three distinct categories. For each there exists already well-defined evaluation metrics used by the wider imaging community which we use for evaluation here. Codes related to all evaluation metrics used in this challenge are also available online\footnote{https://github.com/sharibox/EndoCV2020}.
%
\subsubsection*{Detection and localisation task}
%
Metrics used for multi-class disease detection: 
\begin{itemize}
    \item IoU - intersection over union. This metric measures the overlap between two bounding boxes $A$ and $B$ as the ratio between the overlapped area $A\cap B$ over the total area $A\cup B$ occupied by the two boxes:
    \begin{equation}
        \mathrm{IoU} = \frac{A\cap B}{A\cup B}
    \end{equation}
    where $\cap$, $\cup$ denote the intersection and union respectively. In terms of numbers of true positives (TP), false positives (FP) and false negatives (FN), IoU (aka Jaccard J) can be defined as:
    \begin{equation}
        IoU/J = \frac{TP}{TP+FP+FN}
    \end{equation}
    
    \item mAP - mean average precision of detected disease class with precision (p) defined as $p={\frac {TP}{TP+FP}}$ and recall (r) as $r={\frac {TP}{TP+FN}}$. {This} metric measures the ability of an object detector to accurately retrieve all instances of the ground truth bounding boxes. The higher the mAP the better the performance. Average precision (AP) is computed as the Area Under Curve (AUC) of the precision-recall curve of detection sampled at all unique recall values $(r_1, r_2,...)$ whenever the maximum precision value drops:
    \begin{equation}
        \mathrm{AP} = \sum_n{\left\{\left(r_{n+1}-r_{n}\right)p_{\mathrm{interp}}(r_{n+1})\right\}}, 
    \end{equation}
    % \begin{equation}

    % \end{equation}
    with $p_{\mathrm{interp}}(r_{n+1}) =\underset{\tilde{r}\ge r_{n+1}}{\max}p(\tilde{r})$. Here, $p(r_n)$ denotes the precision value at a given recall value. This definition ensures monotonically decreasing precision. The mAP is the mean of AP over all disease classes $i$ for $N=5$ classes given as
    \begin{equation}
        \mathrm{mAP} = \frac{1}{N}\sum_i{\mathrm{AP}_i}
    \end{equation}
    This definition was popularised in the PASCAL VOC challenge~\cite{pascal-voc-2012}. 
    %The calculation is illustrated in Fig. \ref{fig:detection_metrics_illustration}. 
    The final mAP (mAP$_d$) was computed as an average mAPs for IoU from 0.25 to 0.75 with a step-size of 0.05 which means an average over 11 IoU levels are used for 5 categories in the competition (mAP $@[.25:.05:.75]$ ).
\end{itemize}
Participants were finally ranked on a final mean score $(\mathrm{score_d})$, a weighted score of mAP and IoU represented as:
\begin{equation}
\mathrm{score_d} = 0.6 \times \mathrm{mAP_d} + 0.4 \times \mathrm{IoU_d}
\end{equation}

Standard deviation between the computed mAPs ($\pm \sigma_{score_d}$) are taken into account when the participants have the same $\mathrm{score_d}$. 
%
\subsubsection*{Segmentation task}
%
Metrics widely used for multi-class semantic segmentation of disease classes have been used for scoring semantic segmentation. It comprises of an average score of $F_1$-score (Dice Coefficient), $F_2$-score, precision and recall.

\textbf{Precision, recall, F$_\beta$-scores:}
These measures evaluate the fraction of correctly predicted instances. Given a number of true instances $\#\mathrm{GT}$ (ground-truth bounding boxes or pixels in image segmentation) and number of predicted instances $\#\mathrm{Pred}$ by a method, precision is the fraction of predicted instances that were correctly found, $p=\frac{\#\mathrm{TP}}{\#\mathrm{Pred.}}$ where $\#\mathrm{TP}$ denotes number of true positives and recall is the fraction of ground-truth instances that were correctly predicted, $r=\frac{\#\mathrm{TP}}{\#\mathrm{GT}}$. Ideally, the best methods should have jointly high precision and recall. $\mathrm{F_\beta}$-scores gives a single score to capture this desirability through a weighted ($\beta$) harmonic means of precision and recall, $\mathrm{F_\beta} = (1 + \beta^2) \cdot \frac{{p} \cdot {r}}{(\beta^2 \cdot {p}) + {r}}$.
  
 Participants are ranked on as the increasing value of their semantic performance score given by:
\begin{equation}
\mathrm{score_s} = 0.25* \sum p + r + \mathrm{F_1} + \mathrm{F_2} 
\end{equation}
%
Standard deviation between of each subscores are computed and averaged to obtain the final $\pm \sigma_{score_s}$ which is used during evaluation for participants with same final semantic segmentation score.
\subsubsection*{Out-of-sample generalisation task}
Out-of-sample generalization of disease detection is defined as the ability of an algorithm to achieve similar performance when applied to a completely different institution data. We do not provide any details of this data in this paper as this will be released as a part of test data during the competition. To assess this, participants should apply their trained models on images that were neither included in the training nor test data of the detection and segmentation tasks. Participants will be ranked based on a score gap of generalization defined as:
\begin{equation}
    \mathrm{dev_g} =\mid \mathrm{mAP_d} - \mathrm{mAP_g}\mid
\end{equation}
It is worth noting that the highest $\mathrm{mAP_g}$ with $\mathrm{dev_g} \rightarrow 0$ is required for winning the competition.

{The deviation score $\mathrm{dev_g}$ can be either positive or negative, however, the absolute difference should be very small (ideally, $\mathrm{dev_g} = 0$). The best algorithm should have high $\mathrm{mAP_g}$ and high $\mathrm{mAP_d}$ but a very low $\mathrm{dev_g} (\rightarrow 0$). 
%
%%%
\subsection*{Challenge setup, and ranking procedure}
%%%


==> abstract.tex <==
\clearpage
\newpage
\begin{abstract}
Polyps are well known cancer precursors identified by colonoscopy. However, variability in their size, location and surface makes the identification of their presence and type challenging. Moreover, colonoscopy surveillance and removal of polyps (\textit{referred as polypectomy}) are highly operator dependent procedures. 
There exist a high missed detection rate and incomplete removal of colon polyps due to their variable nature, the difficulties to delineate the abnormality, the high recurrence rates and the anatomical topography of the colon. There have been several developments in realising automated methods for both detection and segmentation of colonic polyps using machine learning. However, the major drawback in most of these methods is their ability to generalise to out-of-sample unseen datasets that come from different center, modality and acquisition system. To test this hypothesis rigorously we curated a multi-center and multi-population dataset acquired from different colonoscopy systems and challenged the computational expert teams to participate in developing robust automated detection and identification solutions. We analyse the segmentation results of the 5 best teams (among 16) and the detection results of the 4 best (among 7) teams which participated at the EndoCV 2021. Our results show that most top ranking teams concentrated on accuracy (i.e., accuracy  $> 80\%$ on overall Dice score on different validation sets) over real-time performance required for clinical applicability. 
\end{abstract}

 

==> conclusion.tex <==
\section*{Conclusion}

==> method.tex <==
\section*{Method summary of the participants}
% To be written by organisers and participants!
% \subsection*{EndoCV2021 Participating teams}
\subsection*{Segmentation Task}
% Type of model overview --->
% Augmentation yes? ---> what
% Epochs, batch size, lr, optimiser, image size, [overall no of parameters (table)], stopping criteria (if any)
% Data split in training (how your dataset was managed)
% Threshold for inference
% Reported training time on their GPU, no of GPU with name
% 
% TODO: Not more than 8-10 lines - please remove results (numbers) but keep how inference was conducted
\begin{itemize}
 \item \textbf{MLC\_SimulaMet:} Thambawita et al.~\cite{thambawita2021divergentnets} developed two ensemble models using well-known segmentation models; namely UNet++~\cite{zhou2018unet++}, FPN~\cite{lin2017feature}, DeepLabv3~\cite{chen2017rethinking}, DeepLabv3+~\cite{chen2018encoder} and novel TriUNet for their DivergentNet ensemble model, and three UNet~\cite{ronneberger2015u} architectures in their TriUNet ensemble model. The novel TriUNet model takes a single image as input, which is passed through two separate UNet models with different randomized weights. The output of both models was then concatenated before being passed through a third UNet model to predict the final segmentation mask. The whole TriUNet network was trained as a single unit. The proposed DivergentNet included five segmentation models that were pre-trained with the training dataset individually before assembling them to DivergetNets using a modified Dice loss function which calculated a loss only for the polyp channel (not for the background channel). 
     
     % Did you train the DivergentNet, i.e., first combine all trained architectures and then train an end-to-end network?
     % What is modified Dice loss (cite if there is a paper on this! if not please explain)
    %Models were trained and tested using the following GPUS: GTX 1080Ti, GTX 1060, V100 and Quadro P6000.
    %Joint Polyp Detection and Segmentation with Heterogeneous Endoscopic Data (http://ceur-ws.org/Vol-2886/)
    
    
   \item \textbf{AIM\_CityU:} Li et al.~\cite{lia2021joint} adopted HRNet~\cite{wang2020deep} as the backbone to maintain the high-resolution representations. To further eliminate noisy information in segmentation predictions and enhance model generalization, the team proposed a low-rank module to distribute feature maps in the high dimensional space to a low dimensional manifold. For the model optimization, various data augmentation strategies, including random flipping, rotation, color shift (brightness, color, sharpness, and contrast) and Gaussian noise, were performed to improve the model generalization further. Cross entropy and dice loss are utilized to optimize the whole model. 

\item \textbf{aggcmab:} Galdran et al.\cite{ galdrana2021multi} improved their previously developed framework cascaded double encoder-decoder convolutional neural network~\cite{galdran2021double} by increasing the encoder representation capability and adapting to a multi-site sampling technique. The first encoder-decoder generates an initial attempt to segment the polyp by extracting features and downsampling spatial resolutions while increasing the number of channels by learning convolutional filters. The output from the first network acts as an input for the second encoder-decoder along with the original image.
    % 2) Experimental design
Cross-entropy loss was minimized using the stochastic gradient descent with a batch-size of 4 and a learning rate of \textit{lr} = 0.01 with rate decay of $1{e}^{–8}$ every 25 epochs. The training images were resized to 640$\times$512, and data augmentation (e.g. random rotations, vertical/horizontal flipping, contrast, saturation and brightness changes) was applied. The average dice score was calculated on the separate validation set, and the best model performance was saved for the testing stage.  
    % 3) Results here
Four versions were generated from the image (i.e. horizontal and vertical flipping), and the average result was calculated on the test set. 
% The final dice score of the model was 81.81$\pm$1.19.
 
\item \textbf{sruniga:} 
  % Sahadev 
%http://ceur-ws.org/Vol-2886/paper4.pdf
% 1) Model description
Ghimire et al.~\cite{ghimirea2021augmentation} suggested a lightweight deep learning-based algorithm to meet the real-time clinical need. The proposed network applies the HarDNet-MSEG~\cite{huang2021hardnet} as the backbone network as it has a low inference speed due to reduced shortcuts. Moreover, they proposed an augmentation strategy that encourages the model to learn semantic features from different variations that helps to generalize the model. The data augmentation is applied according to a certain probability.  
% 2) Experimental design
For training the model, the dataset was split into 80\% training and 20\% validation using adam optimizer and setting the learning rate \textit{lr}=0.00001 for all the experiments. Images were resized to 352$\times$352, and data augmentation has been applied according to the proposed algorithm by the team.  
% 3) Results here
To test the performance of the model, the results are compared with different state-of-the-art segmentation methods such as UNet~\cite{ronneberger2015u}, ResUNet~\cite{zhang2018road}, UNet++~\cite{zhou2018unet++} and ResUNet++~\cite{jha2019resunet++}. The HardNet achieved the best performance with and without applying the augmentation. The final results showed Jaccard Index (mIoU) and DSC of 0.8485, and 0.8923 respectively, without data augmentation. With the data augmentation, there was a slight improvement in the results, and the proposed approach obtained the DSC of 0.8649 and mIoU of 0.9124. 



\item \textbf{Mah\_UNM:}
    % 1) Model description
Haithami et al.~\cite{haithamia2021embedded} proposed modifying the SegNet~\cite{badrinarayanan2017segnet} by embedding Gated recurrent units (GRU) units~\cite{cho2014learning } within the convolution layers to improve its performance in segmenting polyps.  The suggested SegNet employs the VGG16 as the backbone network, and one GRU unit was used before the last convolution layer at each stage to extract contextual information. The output from each GRU unit was concatenated with the input feature map and passed to the next stage. The total number of stages in the proposed network was five for both the encoder and the decoder. 
% 2) Experimental design
The hyperparameters were set as the original SegNet with learning rate \textit{lr}=0.005 and batch size of 4. The multiplicative factor of “gamma=0.8” was used for the learning rate decay with adam optimizer and weighted cross-entropy loss. The provided dataset was split into 80\% training and 20\% validation.  
% 3) Results here
Four experiments were held to evaluate the effect of adding the GRU unit to the original SegNet. The results of the four experiments were compared with the original SegNet architecture. The proposed method obtained DSC of 0.1922 and mIoU of 0.1063. 


\item \textbf{HoLLYS\_ETRI:} Hong et al.~\cite{honga2021deep} proposed an ensemble inference model based on 5-fold cross-validation to improve the performance of polyp detection and segmentation.  The Mask R-CNN was used to generate the output segmentation mask. Ensemble inference was used to generate the final segmentation mask by averaging the results from the 5 models. After averaging the masks, if the inference results were greater than the threshold (0.6) then the output mask is considered as a polyp otherwise was counted as a background. Data augmentation was performed based on the techniques provided in Detectron2 (i.e. RandomBrightness, RandomContrast, RandomSaturation, and RandomLighting), in addition to, random crop and flipping of the images. The model was trained for 50,000 steps and checkpoints were save for every 1,000 steps. The stochastic gradient descent (SGD) was used as an optimizer with learning rate \textit{lr}=0.001 that changes with a warm-up scheduler.
  % The proposed model scored 0.7423$\pm$ 0.2839 for the segmentation task

   
\item \textbf{NDS\_MultiUni:} Tomar et al.~\cite{tomara2021improving} suggested building a cascaded ensemble model made of MultiResUNet \cite{ibtehaz2020multiresunet} architectures. The MultiResUNet is composed of four encoders, decoders and a connecting bridge.  The encoder extract features from the input image, which is fed to the decoder. The features from the decoder are upsampled and contacted with the feature maps from the skip connection. The input image is fed to four different MultiResUNet models in the proposed model, and each model generates an output mask. Afterwards, the four predicted outputs are averaged together to produce the final segmentation mask. In order to train the different subsets of the dataset from the five centres are trained by one of the four MultiResUNet models.  Each model is trained for 100 epochs with the same setting of hyperparameters. The input images were resized to 256$times$256 with a batch size of 8, binary cross-entropy as loss function and using adam optimizer. The learning rate is set to \textit{lr}=1\textit{e}-3 and using the Reduce LROnPlateau callback. %The experimental results showed that the ensemble model obtained a dice score of 0.6172 $\pm$ 0.0778.
   
\item \textbf{YCH\_THU:} Yu et al.~\cite{yua2021parallel} aimed to enhance the Parallel Reverse Attention Network (PraNet) \cite{pavlatos2016linguistic}. The proposed methods extract multi-level features from colonoscopy images utilizing a parallel res2Net-based network. The high-level features and output of the partial decoder were put parallel into a reverse attention component in order to adjust segmentation to accurate results. Moreover, the segmentation results are post-processed to remove uncertain pixels and enhance the boundary. The images were resized to 512$\times$512 and the dataset was split into 80\% training and 20\% validation. The model was trained for 300 epochs with batch size 18 and learning rate \textit{lr}=1\textit{e}-4 which was reduced every 50 epochs. 
%The model was trained and tested on different datasets to ensure generalizability. The best performance was achieved y the proposed model on the EndoCv21 dataset with an accuracy of 0.9342. 

\end{itemize}

\subsection*{Detection Task}
\begin{itemize}
    \item \textbf{AIM\_CityU:}~\cite{lia2021joint} The authors used one-stage anchor-free FCOS~\cite{tian2019fcos} as the baseline detection algorithm and adopted ResNeXt-101-DCN~\cite{zhu2019deformable} with FPN as their final feature extractor. To handle the two kinds of inconsistency that appeared in the endoscopic dataset, thus Optimization Inconsistency (OI) and  Data Inconsistency (DI), the authors adopted GFL v2~\cite{gflv2} to optimize classification and regression jointly and Adaptive Training Sample Selection (ATSS)~\cite{zhang2020bridging} strategy to improve the generalization abilities. For the model optimization, both online (random flipping and multi-scale training) and offline (random rotation, gamma contrast, and brightness transformation, etc.) data augmentation strategies are performed to improve the model generalization. Besides, the authors performed instance-level over-sampling in ATSS to increase the variance of polyp samples. In the inference stage, they reduced the NMS threshold to 0.01 and increased the classification score threshold to 0.3 to obtain better polyp detection results.


    \item \textbf{HoLLYS\underline{ }ETRI:}~\cite{honga2021deep}
    The authors used a mask R-CNN~\cite{he2017mask} for detection and segmentation task. All the weights were initialized with pre-trained weights using the COCO dataset.
    An ensemble learning method based on 5-fold cross-validation was used to improve the generalization performance. While training a single mask R-CNN, the data acquired from all data centers were not used. Instead, only the data acquired from data from four centers were used for training and, the data from remained center was used for validation. 
    When the model to be learned changed, so did the center of data used for validation.
    Ensemble inference was performed by combining the inference results of 5 models. For the detection task, Weighted box fusion technique~\cite{solovyev2021weighted} was used to combining results of detection. For segmentation task, segmentation masks from 5 models were averaged and the area where over than score 0.6 was considered as polyp area.
    
    \item \textbf{JIN\_ZJU:}~\cite{gana2021detection} The authors used the YoloV5 \cite{yolov5}  as the baseline detection algorithm after comparing three state-of-the-art object detection methods: EfficientDet, ScaledYOLOv4 and YOLOv5. To improve the performance of the standard Yolov5, different data augmentation methods have been applied such as hue adjustment, saturation adjustment, value adjustment, rotating, translation, scaling, up-down flipping, left-right flipping, mosaic and mixup.
    
    \item \textbf{Gece\_vision:} \cite{polat2021polyp}
    % Normalization, rescaling by keeping aspect ratio => EfficientDet (D0, D1, D2, D3) => non-max suppression, bootstrap aggregation for ensemble, weighted box fusion for merging different predictor results
    % 1) Model description
    The authors propose an ensemble-based polyp detection architecture using the EfficientDet \cite{tan2020efficientdet} as the base model family with EfficientNet \cite{tan2019efficientnet} as backbone network.  The Bootstrap aggregating (bagging) \cite{breiman1996bagging} is utilized to aggregate different versions of the predictors (EfficientDet D0, D1, D2, D3) which are trained on bootstrap replicates of the training set.
    % 2) Experimental design (4:1 fold???)
    Each model from the EfficientDet family is trained on separate folds and uses 75\% of the samples in that fold for training and 25\% for validation. The bounding boxes generated individually by each model are then merged using weighted box fusion~\cite{solovyev2021weighted}. In order to increase the variance and improve generalization capability of the model, data augmentation have been used (i.e., scale jittering with 0.2-2.0, horizontal flipping, and rotating between 0°-360°). Adam optimizer and the scheduling learning rate have been with decrease factor of 0.2 whenever validation loss did not change in the last 10 epochs. 
    % 3) Results here (only put EndoCV2021 <--->)
    The model was trained and tested on both the EndoCV2021. The performance was evaluated on both datasets using  in- and out-of-distribution manner. The weighted box fusion of different models results in increased performance.  The best overall detection performance on both test sets is obtained when the proposed bagging ensemble approach is used with results of 0.906 $mAP\_50$ for EndoCV2021.
 \end{itemize}
 
 
\begin{table*} [!t]
\footnotesize
\centering
\caption{{Summary of the participating teams \textbf{Detection task} for EndoCV2021 Challenge}. All test was done on NVIDIA V100 provided by the organisers.}
\begin{tabular}{p{2cm}|p{1.8cm}|p{2cm}|p{1cm}|p{1.2cm}|p{0.5cm}|p{1.4cm}|p{1.1cm}|p{1.5cm}}
\toprule
\bf Team Name &\bf Algorithm & \bf Backbone &\bf Nature  &\bf \begin{tabular}[l]{@{}c@{}}
    Choice  \\ Basis\end{tabular} & \bf \begin{tabular}[l]{@{}c@{}}
    Data  \\ Aug.\end{tabular} & \bf \begin{tabular}[l]{@{}c@{}}
    Loss  \\ function\end{tabular}& \bf Optimizer&\bf Code\\  \midrule  \midrule
AIM\_CityU \cite{lia2021joint} & ResNeXt-101-DCN & FPN  & ATSS & \begin{tabular}[l]{@{}c@{}}
    Accuracy  \\
      speed 
\end{tabular}  & No &  Generalized Focal Loss & SGD  &CityU-AIM-Group/EndoCV-2021 \\  %\hline  %(lr, batch size, image size, normalization, Optimizer

% \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Endocv Detection}}} 

 HoLLYS\underline{ }ETRI \cite{honga2021deep} & Mask R-CNN  &  FPN & Ensemble & Accuracy++  & No &Smooth L1   & SGD &EndoCV2021/detectron\\ %\hline

JIN\_ZJU \cite{gana2021detection}  & YoloV5 & CSPdarknet+SPP & Ensemble & speed++ & Yes & BECLogits Loss & SGD & /GTYuantt/EndoCV2021_yolov5\\ %\hline
% Jin Loss  BCEcls loss; GIOU Loss
gece\_vision \cite{polat2021polyp} & EfficientDet   & EfficientNet   & Ensemble & Accuracy & Yes & - & Adam &GorkemP/EndoCV2021-EfficientDet-Pytorch\\ %\hline
% &Team Name &  &   & &  & No &  & & &\\ %\hline

% &Team Name &  &   & &  & No &  & & &\\ %\hline
% &Team Name &  &   & &  & No &  & & &\\ %\hline


\bottomrule
\end{tabular}
 \label{table:challenge_summary}
\end{table*}

% Definition of basis-of-choice: Accuracy, robustness, speed, speed++, Accuracy++
\begin{table*} [!t]
\footnotesize
\centering
\caption{{Summary of the participating teams algorithm for \textbf{segmentation task} Endocv2021 Challenge}.}
\begin{tabular}{p{2.3cm}|p{2cm}|p{1.6cm}|p{1cm}|p{1.2cm}|p{0.5cm}|p{1.3cm}|p{1.2cm}|p{1.5cm}}
\toprule
\bf Team Name &\bf Algorithm & \bf Backbone &\bf Nature  &\bf \begin{tabular}[l]{@{}c@{}}
    Choice  \\ Basis\end{tabular} & \bf \begin{tabular}[l]{@{}c@{}}
    Data  \\ Aug.\end{tabular} & \bf \begin{tabular}[l]{@{}c@{}}
    Loss  \\ function\end{tabular}& \bf Optimizer &\bf Code\\  \midrule  \midrule
MLC\_SimulaMet~\cite{thambawita2021divergentnets} &DivergentNet  &  TriUNet  & Encoder& Accuracy & No & \begin{tabular}[l]{@{}c@{}}
    Binary  \\
      DSC loss 
\end{tabular}& Adam & vlbthambawita/divergent-nets\\ %\hline

AIM\_CityU~\cite{lia2021joint} & HRNet & HRNet  & Low-Rank Module &Accuracy  & Yes &  cross entropy loss + dice loss & SGD & CityU-AIM-Group/EndoCV-2021\\ %\hline

aggcmab \cite{ galdrana2021multi} & DPN92-FPN & DPN92-FPN  & encoder-decoder& Accuracy & Yes &Binary Cross-Entropy   & SGD& agaldran/endocv21\\ %\hline
sruniga \cite{ghimirea2021augmentation} & HarDNet68  & HarDNet68   &CNN & Accuracy++& No &  & Adam& SahadevPoudel/HarDNet-MSEG \\ %\hline
HoLLYS\_ETRI \cite{honga2021deep}& Mask R-CNN & ?  & Ensemble & Accuracy++ & Yes & Smooth L1   & SGD  & EndoCV2021/detectron \\ %\hline
YCH\_THU \cite{yua2021parallel} & PraNet  &  res2Net   & encoder-decoder &Accuracy, Speed  & No &  Weighted IOU loss + Weighted  BCE loss &Adam  & kirtsy/Polyp-Segmentation--endoCV2021
\\ %\hline
NDS\_MultiUni \cite{tomara2021improving} &MultiResUnet  & ResUnet  & Ensemble& Accuracy  & No & Binary Crossentropy & Adam & NA \\ %\hline
Mah\_UNM \cite{haithamia2021embedded} & SegNet & VGG16  & GRU & Accuracy++ & No & Cross Entropy & Adam& mss3331/HandSeg \\ %\hline
\bottomrule
% https://github.com/
\end{tabular}
 \label{table:challenge_summary}
\end{table*}
% TODO: rewrite/contract @ Debesh
% \subsection*{Experimental setup}
% \subsection*{Evaluation metrics}
% % What will reader find in the evaluation metric section? What is different/new here?
% https://github.com/sharibox/EndoCV2021-polyp_det_seg_gen
% \subsection*{Baseline experimental setup and design}

% \section*{Discussion}

% \section*{Conclusion}



==> supplimentaryFile1.tex <==
\section{EAD2019 challenge leaderboard}
\begin{itemize}
    \item Summarize in words regarding numbers and leaderboard and methods
    \item Summary table (Sharib will do this)
    \item Link all to Suppl. Material 2 
    \begin{itemize}
        \item Leaderboard
        \item Algorithms in detail: 3-4 short paragraphs per method (till 6 top methods for detection and 6 for segmentation)
        \item Suppl. Note
        \item Executable versions if available
    \end{itemize}
\end{itemize}

==> takeout.tex <==


% \bf \thead{Challenge Name} &\bf Organ &\bf Modality  &\bf Findings & \bf Size & \bf \thead{Dataset\\Availability} \\ \midrule

% \thead{Automatic Polyp Detection\\in Colonoscopy videos 2015\cite{bernal2017comparative}} & Colon & WL & Polyps & \thead{$808$ images\\ \& $38$ videos} & By request \\ %\hline

% \text{Medico task} 2017~\cite{riegler2017multimedia} & Entire \ac{GI} & WL & \thead{Polyps, esophagitis, ulcerative colitis,\\ z-line, pylorus, cecum, dyed polyp,\\ dyed resection margins, stool} & $8,000$ images & Open academic \\ %\hline

% GIANA 2017~\cite{gianadataset2017} & Colon & WL & Polyps \& angiodysplasia & \thead{$3462$ images\\ \& $38$ videos} & By request \\ %\hline 

% GIANA 2018~\cite{angermann2017towards,bernal2018polyp} & Colon & WL, WCE  & Polyps \& small bowel lesions & \thead{$8,262$ images\\ \& $38$ videos}  & By request \\ %\hline 

% Medico task 2018~\cite{pogorelov2018medico} & Entire \ac{GI} & \thead{WL} & \thead{Blurry-nothing, colon-clear, dyed-lifted-polyp,\\ dyed-resection-margin, esophagitis, instrument,\\ normal-cecum, normal-pylorus, normal z-line,\\ out-of-patient, polyp, retroflex-rectum,\\ retroflex-stomach, stool-inclusion, stool-plenty,\\ ulcerative-colitis}  &$14,033$ images & Open academic\\ %\hline 

% EAD 2019~\cite{ali2019endoscopy} & \thead{Entire \ac{GI}\\ \& bladder} & \thead{NBI, WL,\\ FL, WCE} & \thead{Blur, bubbles, contrast, imaging \\artefact,  saturation, specularity, instrument} & $2,192$ images &  Open academic\\ %\hline 

% \thead{BioMedia grand\\challenge 2019\cite{hicks2019acm}} & Entire \ac{GI} & \thead{WL} & \thead{Blurry-nothing, colon-clear, dyed-lifted-polyp,\\ dyed-resection-margin, esophagitis, instrument,\\ normal-cecum, normal-pylorus, normal Z-line,\\ out-of-patient, polyp, retroflex-rectum,\\ retroflex-stomach, stool-inclusion, stool-plenty,\\ ulcerative-colitis} & $14,033$ images & Open academic \\ %\hline

% EAD 2020~\cite{ali2019endoscopy} & \thead{Entire \ac{GI}\\ \& bladder} & \thead{NBI, WL,\\ FL, WCE} & \thead{Blur, bubbles, blood, contrast, imaging \\artefact,  saturation, specularity,  instrument} & $2,916$ images &  Open academic\\ %\hline 

% EDD 2020~\cite{ali2020endoscopy} & Entire \ac{GI} & \thead{NBI, WL} & \thead{Barrett's esophagus, high-grade dysplasia, \\suspicious (low-grade), polyp, cancer} & $386$ images & Open academic\\ 
% \bottomrule
% \end{tabular}
% \caption{Overview of \ac{GI} endoscopy challenges. Here, WL = White Light Endoscopy, NBI = Narrow Band Imaging, WCE = \acf{WCE}, FL = Fluorescence Endoscopy. The total number of images and videos offered at different task are sumed and presented in 'Size' class.}
% \label{tab:challengeoverview}
% \end{table*}
